Dual-Route Top-K Retrieval with 1v1 VLM Reranking for the CoVR-R

We describe \emph{Dual-Route Top-K Retrieval with 1v1 VLM Reranking} for the CoVR-R challenge. The method treats composed video retrieval as two coupled problems: finding a sufficiently complete top-k candidate set, and then safely deciding whether any candidate should replace a strong current top-1. We first improve the reasoning/text seed with a VLM slot selector over existing candidates, without introducing DFN visual retrieval. We then add a visual route from contact-sheet embeddings using DFN-H/DFN-L. The routes are merged into a top-10 candidate set, after which a VLM final reranker performs conservative 1v1 comparisons between the current top-1 and each challenger. On the hidden test split, the final system reaches 95.28 R@1, 97.47 R@5, 98.48 R@10, and 99.66 R@50. The main lesson is that CoVR-R benefits more from recall-selection decoupling than from broad text reranking or direct multi-candidate VLM classification.

==> tables/ablation_summary.tex <==
\begin{table*}[t]
\centering
\caption{Ablations supporting the dual-route and 1v1 reranking design.}
\label{tab:ablations}
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{p{0.19\linewidth}p{0.38\linewidth}p{0.35\linewidth}}
\toprule
Ablation module & Intervention & Observation \\
\midrule
Text-only reranking & Multi-description RRF and edit-type routing over cached captions/reasoning. & Negative; text matching changed too many top-1 and top-50 rankings. \\
Top-1 VLM slot selection & Score existing candidates with structured slot evidence before DFN visual retrieval. & Positive for R@1 while keeping R@5/R@10/R@50 fixed. \\
Top1-preserving visual injection & Merge visual-route candidates into top10 while preserving the seed top-1. & R@5/R@10/R@50 improved sharply, proving recall was still available. \\
1v1 final reranking & Compare each merged top2--top5 challenger against the current top-1. & R@1 improved without changing top5/top10/top50 sets. \\
Distant-rank promotion & Promote top6--top50 candidates directly after visual audit. & Negative; distant candidates were visually plausible but risky for top-1. \\
Consensus filtering & Require two structured VLM reviewers to agree on a zero-fatal challenger. & Small but clean R@1 gain; final best result. \\
\bottomrule
\end{tabular}
\end{table*}

